Adding more data does not always help: A study in medical conversation summarization with PEGASUS

Medical conversation summarization is integral in capturing information gathered during interactions between patients and physicians. Summarized conversations are used to facilitate patient hand-offs between physicians, and as part of providing care in the future. Summaries, however, can be time-consuming to produce and require domain expertise. Modern pre-trained NLP models such as PEGASUS have emerged as capable alternatives to human summarization, reaching state-of-the-art performance on many summarization benchmarks. However, many downstream tasks still require at least moderately sized datasets to achieve satisfactory performance. In this work we (1) explore the effect of dataset size on transfer learning medical conversation summarization using PEGASUS and (2) evaluate various iterative labeling strategies in the low-data regime, following their success in the classification setting. We find that model performance saturates with increase in dataset size and that the various active-learning strategies evaluated all show equivalent performance consistent with simple dataset size increase. We also find that naive iterative pseudo-labeling is on-par or slightly worse than no pseudo-labeling. Our work sheds light on the successes and challenges of translating low-data regime techniques in classification to medical conversation summarization and helps guides future work in this space. Relevant code available at \url{https://github.com/curai/curai-research/tree/main/medical-summarization-ML4H-2021}.

==> sections/dataset.tex <==
\section{Dataset}
\label{sec:dataset}

To compile our dataset, we follow the procedure described in \cite{chintagunta-etal-2021-medically} in collecting chat conversations between physicians and patients from a tele-medicine platform. We 

The end 

Our dataset was compiled oFor our task of medical conversation summarization

Our dataset + relationship to GPT-3 paper

Figure showing example of our data

% \begin{table*}[!ht]
%     \centering
%     \begin{tabular}{ll}
%     \toprule
%     \textbf{Snippet} & \textbf{Summary} \\
%     \midrule
%     \textbf{Physician:} Thanks for sharing. What about the back pain? Doing better with that? \\
%     \textbf{Patient:} Still there every once in a while, but not daily \\
%     \textbf{Physician:} Good to know things look better! \\
%     \textbf{Patient:} Thank you! \\
%         % Dropout &  0.1 \\ & 0.5 \\
%         % \midrule
%         % Pseudo-labeling strategy & None \\ 
%         %                          & Top 1\% \\
%         %                          \midrule
%         % Human-labeling strategy  & None \\ 
%         %                          & Bottom 1\% \\  
%         %                          & Middle 1\% \\  
%         %                          & Random 1\% \\ 
%         %                          \midrule
%         % Starting number of samples  & 100 \\ 
%         %                          & 250 \\  
%         %                          & 500 \\  
%         %                          & 750 \\  
%         %                          & 1000 \\  
%         %                          & 1250  \\
%     \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:Experiments}
% \end{table*}
